Toric degenerations and Newton-Okounkov bodies

In recent times, a wide variety of combinatorics has been introduced in order to solve problems from algebraic geometry. Newton-Okounkov bodies and tropical geometry are two such combinatorial theories. As shown by Kaveh and Manon, there is a certain correspondence between these two. Building on this correspondence, and exploiting the link of both theories to toric degenerations, Harada and Escobar obtained their wall-crossing result for prime cones. This result states that moving between two adjacent prime maximal cones in a tropical variety corresponds to a mutation between the associated Newton-Okounkov bodies of these cones. In this thesis, we provide a method for applying the wall-crossing result to non-prime cones. Our approach uses a procedure developed by Bossinger, Lamboglia, Mincheva and Mohammadi in order to compute an embedding which changes a tropical variety in such a way that a non-prime cone becomes prime. Assuming that adjacent cones stay adjacent, the wall-crossing result can then be applied in this new embedding. Building on computations by Clarke, Mohammadi and Zaffalon, we show that for Gr(3,6), this approach works. We compute the new embedding and its tropicalization in this case, and study the relation between cones in the new embedding and the original embedding.

==> chapters/abstract/abstract.tex <==
% !TeX root = ../../thesis.tex
\chapter{Abstract}                                 \label{ch:abstract}
In recent times, a wide variety of combinatorics has been introduced in order to solve problems from algebraic geometry.
Newton-Okounkov bodies and tropical geometry are two such combinatorial theories. As shown by Kaveh and Manon, there is a certain correspondence between these two. Building on this correspondence, and exploiting the link of both theories to toric degenerations, Harada and Escobar obtained their wall-crossing result for prime cones. This result states that moving between two adjacent prime maximal cones in a tropical variety corresponds to a mutation between the associated Newton-Okounkov bodies of these cones.\\
In this thesis, we provide a method for applying the wall-crossing result to non-prime cones. Our approach uses a procedure developed by Bossinger, Lamboglia, Mincheva and Mohammadi in order to compute an embedding which changes a tropical variety in such a way that a non-prime cone becomes prime. Assuming that adjacent cones stay adjacent, the wall-crossing result can then be applied in this new embedding.\\ 
Building on computations by Clarke, Mohammadi and Zaffalon, we show that for $\Gr(3,6)$, this approach works. We compute the new embedding and its tropicalization in this case, and study the relation between cones in the new embedding and the original embedding.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/preface/preface.tex <==
% !TeX root = ../../thesis.tex
\chapter*{Acknowledgements}                                  \label{ch:Acknowledgements}

I want to thank Prof. Dr. F. Mohammadi for introducing me to the fascinating subjects of tropical geometry and Newton-Okounkov bodies, and for providing me with numerous opportunities to learn and improve myself. My sincerest gratitude goes out to F. Zaffalon for her exceptional guidance, her clear answers to my abundant questions and all her extremely helpful feedback.\\
I am deeply grateful to my parents for their unwavering faith in me. Without your constant push for me to strive for greater heights, I would not have made it here. Lastly, my thanks go out to my girlfriend, my brothers and my friends, for their support and for their patience in listening when things seemed overwhelming.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> mycoverpage.tex <==
% Redefine in this file the commands to generate the front and back cover:
%
%   \makefrontcovergeneral{xskip}{clearpage}
%   \makebackcovergeneral{xskip}{clearpage}
%
% You can start from their definition in adsphd.cls. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% My own cover page
%\makeatletter

%% \renewcommand{\makefrontcovergeneral}[2]{%
%%   %
%%   % Create header
%%   \frontcoverheader{#1}
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Title, subtitle, authorname, text and date can be moved around.
%%   % Change the textblock* commands below. 
%%   %
%%   % Syntax of textblock environment:
%%   % 
%%   %   \begin{textblock*}{width}(xpos,ypos)
%%   %     ...
%%   %   \end{textblock*}
%%   % 
%%   % !! Make sure not to remove the '+#1' part!!!
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Place the title
%%   \begin{textblock*}{120mm}(17.5mm+#1,89.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \raggedright\selectfont\LARGE\sffamily\textbf{\@title}
%%   \end{textblock*}
%%   %
%%   % Place the subtitle
%%   \begin{textblock*}{120mm}(17.5mm+#1,92.0mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \Large\sffamily{\@subtitle}
%%   \end{textblock*}
%%   %
%%   % Place the author name
%%   \begin{textblock*}{120mm}(17.5mm+#1,109.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \Large\sffamily\@authorf\ \MakeUppercase\@authorl
%%   \end{textblock*}
%%   %
%%   %\begin{textblock}{120}(0,115)
%%   \begin{textblock*}{120mm}(17.5mm+#1,132.0mm)
%%   \textblockcolour{}
%%   \includegraphics*{image/coverfigure}
%%   \end{textblock*}
%%   %
%%   % Place the misc text
%%   \begin{textblock*}{60mm}(96.5mm+#1,187.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   {\small\sffamily Dissertation presented in partial\\
%%   fulfillment of the requirements for\\
%%   the degree of Doctor\\
%%   in \@degree}
%%   \end{textblock*}
%%   %
%%   % Place date
%%   \begin{textblock*}{160mm}(0mm+#1,221.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \begin{center} {\small\sffamily\@date }\end{center}
%%   \end{textblock*}
%%   
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Add footer
%%   \frontcoverfooter{#2}
%% 
%% }

%\makeatother

